Refutation of K2-256b and Rejection of 130 Unconfirmed Transiting Planet Candidates with Gaia DR3 NSS

Much of the exoplanet discovery efforts over the next several years are largely tasked with finding candidates for the upcoming Ariel mission. This is a role that TESS is well-suited for. Radial velocity follow-up is needed to confirm the planetary nature of these systems, as many of its planet candidates turn out to be eclipsing binary systems with small stellar secondaries. Focused Doppler follow-up to obtain these radial velocities is expensive. The Gaia mission's radial velocity measurements on its target stars are not adequately precise for a general search for orbiting planetary companions. While the RV data has yielded thousands of spectroscopic binary systems, only an extreme minority of these reach into the planetary-mass regime. Nonetheless, they do detect eclipsing binary systems that can masquerade as transiting hot Jupiters. In this work, we compare the Gaia DR3 Non-Single Stars catalogue to the current planet candidate list from TESS and determine several of these candidate planetary systems are actually eclipsing binaries. We find $\sim130$ eclipsing binaries among the TOI and EPIC lists that do not appear to be in the literature, including the previously statistically validated planet K2-256 b. This work illustrates the usefulness of \textit{Gaia} to exoplanet validation efforts and will help guide follow-up efforts for discovering new transiting planets for the Ariel mission by avoiding misdirecting valuable telescope time.

==> NewBlends.tex <==
\clearpage
\begin{deluxetable*}{rrcccllr}
\centering
\tablecolumns{8}
\tablecaption{Candidate Transiting Planets Rejected as Blends with Known Eclipsing Binaries}
\tablehead{\colhead{Gaia DR3 ID (EB)} & \colhead{Period [d]} & \colhead{ecc}& \colhead{$\omega [\degr]$} & \colhead{$K_\text{RV}$ [km s$^{-1}$]} & \colhead{$T_\text{peri}$ JD} & \colhead{$T_\text{transit}$ JD} & \colhead{Candidate Planet}}
\startdata
659288410630096000&$6.76224\pm0.00068$&$0.04\pm0.03$&$290.7\pm29.7$&$65.328\pm1.265$&$2457386.024\pm0.56$&2457142.603&EPIC 211808055\\
659847065615319936&$635.30116\pm4.91832$&$0.03\pm0.01$&$87.3\pm27.3$&$6.117\pm0.072$&$2457087.524\pm49.42$&2458097.30654&EPIC 211839462\\
6769386779452266240&$43.09315\pm0.01971$&$0.21\pm0.03$&$56\pm10.4$&$26.364\pm1.451$&$2457386.649\pm1.185$&2457303.7453&EPIC 214912104\\
3693923014184650496&$5.51872\pm0.00018$&$0.01\pm0.01$&$122.1\pm70.3$&$45.074\pm0.487$&$2457387.835\pm1.078$&2457586.5247&K2-256\\
3220802537980446848&$4.72878\pm0.00051$&$0.17\pm0.12$&$248.3\pm16.2$&$39.137\pm5.560$&$2457387.221\pm0.239$&2459196.648037&TOI-484\\
3285409673726608768&$2.96835\pm0.00011$&$0.06\pm0.02$&$341.1\pm15.9$&$16.529\pm0.272$&$2457389.074\pm0.13$&2458441.29935&TOI-951\\
5254794943714396800&$5.54829\pm0.00093$&$0.08\pm0.1$&$246.4\pm37.4$&$18.488\pm1.180$&$2457388.179\pm0.618$&2459328.032732&TOI-1888\\
3291551648758101248&$6.48369\pm0.00077$&$0.25\pm0.05$&$343.5\pm7.3$&$21.855\pm1.158$&$2457391.633\pm0.131$&2458444.08008&TOI-2473\\
5808849641863958528&$4.72573\pm0.00084$&$0.24\pm0.09$&$332.7\pm19.5$&$20.877\pm1.704$&$2457390.585\pm0.223$&2459386.781009&TOI-4420\\
\vspace{-0.3cm}
\enddata
\tablecomments{New EBs Matches between Gaia DR3 NSS SB1 and candidate transiting planet systems.}
\end{deluxetable*}

==> NewEBs.tex <==
\begin{deluxetable*}{rrcccllr}
\tablecolumns{8}
\tablecaption{Gaia Parameters for Eclipsing Binaries Masquerading as Planets Identified in This Work}
\tablehead{\colhead{Gaia DR3 ID} & \colhead{Period [d]} & \colhead{ecc}& \colhead{$\omega [\degr]$} & \colhead{$K_\text{RV}$ [km s$^{-1}$]} & \colhead{$T_\text{peri}$ JD} & \colhead{$T_\text{transit}$ JD} & \colhead{Match}}
\startdata
3798898062211776256&$36.70186\pm0.02628$&$0.16\pm0.04$&$317.2\pm13.9$&$14.014\pm0.452$&$2457394.517\pm1.451$&2456819.743&EPIC 201516974\\
600099122725424768&$14.44576\pm0.00675$&$0.29\pm0.03$&$139.8\pm7.8$&$42.685\pm1.708$&$2457395.475\pm0.283$&2457149.36754&EPIC 211342524 \\
601790961883658112&$5.03558\pm0.00049$&$0.23\pm0.05$&$304.4\pm11.5$&$27.621\pm1.877$&$2457390.908\pm0.151$&2457141.80767&EPIC 211418290\\
602552128870918144&$5.17615\pm0.0001$&$0.01\pm0.00$&$230.6\pm32.7$&$50.062\pm0.240$&$2457389.305\pm0.469$&2457144.49837&EPIC 211424769\\
604460473035451904&$11.10973\pm0.0029$&$0.21\pm0.03$&$239.8\pm8.5$&$50.316\pm1.285$&$2457389.247\pm0.231$&2458101.75989&EPIC 211452175\\
611323517241144576&$20.90523\pm0.01414$&$0.12\pm0.04$&$344.8\pm20.4$&$10.289\pm0.454$&$2457398.153\pm1.194$&2458114.64853&EPIC 211830293 \\
635409251456055168&$19.63571\pm0.00414$&$0.38\pm0.03$&$100.7\pm4$&$30.661\pm1.033$&$2457388.068\pm0.172$&2457152.387959&EPIC 211886472 \\
663154156074506752&$3.69672\pm0.00007$&$0.10\pm0.01$&$113\pm3.6$&$63.150\pm0.512$&$2457389.479\pm0.037$&2458095.87322&EPIC 212024647\\
637075282154501760&$23.69902\pm0.01602$&$0.31\pm0.08$&$246.5\pm7.6$&$38.619\pm3.626$&$2457381.928\pm0.409$&2458118.09327&EPIC 212033577 \\
665412587317415296&$2.23023\pm0.00038$&$0.04\pm0.09$&$277.5\pm97.6$&$39.664\pm2.886$&$2457388.246\pm0.631$&2458096.61073&EPIC 212039539\\
3579529686991039360&$16.77208\pm0.00425$&$0.11\pm0.04$&$133.1\pm20.1$&$10.833\pm0.482$&$2457385.451\pm0.893$&2457585.7609&EPIC 228729473\\
3408649117423934208&$6.76995\pm0.00253$&$0.01\pm0.07$&$233.3\pm254.3$&$22.786\pm1.639$&$2457388.887\pm4.741$&2457826.768729&EPIC 247281516\\
3876036185948161792&$4.98221\pm0.00016$&$0.02\pm0.02$&$193.1\pm42$&$39.944\pm0.688$&$2457387.84\pm0.58$&2457907.544262&EPIC 248740905\\
6238897432936164736&$5.11791\pm0.00141$&$0.08\pm0.1$&$176.8\pm67.4$&$26.848\pm2.732$&$2457388.948\pm0.967$&2457991.898239&EPIC 249239123\\
630850328354376320&$19.60855\pm0.01464$&$0.47\pm0.08$&$45.3\pm6.8$&$20.186\pm3.151$&$2457380.718\pm0.413$&2458107.28569&EPIC 251292838\\
4720986721294105216&$14.15451\pm0.00108$&$0.29\pm0.01$&$293.3\pm2.8$&$24.110\pm0.358$&$2457387.93\pm0.087$&2459128.64364&TOI-156\\
6804708139515008640&$7.76531\pm0.00339$&$0.09\pm0.06$&$41.1\pm52.7$&$13.438\pm1.298$&$2457391.928\pm1.055$&2459078.393053&TOI-162\\
5270358663889956480&$4.81702\pm0.00035$&$0.06\pm0.03$&$138.9\pm22.1$&$18.964\pm0.501$&$2457388.186\pm0.293$&2459165.546503&TOI-184\\
4919562197762515456&$224.790592\pm0.89777$&$0.35848\pm0.08394$&$265.1\pm12.2$&$17.644\pm0.648$&$2457424.26\pm6.518$&2458326.64586&TOI-289\\
3262082160152897408&$7.0118\pm0.00028$&$0.01\pm0.02$&$135.7\pm110.8$&$11.434\pm0.171$&$2457389.934\pm2.147$&2459163.41477&TOI-416\\
2988427421239442432&$3.60469\pm0.00103$&$0.06\pm0.1$&$119.6\pm110$&$10.693\pm1.273$&$2457387.905\pm1.116$&2458440.31143&TOI-425\\
4676885550423032064&$4.42917\pm0.00006$&$0.01\pm0.01$&$231.6\pm62.7$&$52.004$&$2457386.727\pm0.771$&2460144.833166&TOI-459\\
5538255324833781888&$22.61198\pm0.01835$&$0.35\pm0.07$&$263.9\pm10.5$&$19.621\pm2.087$&$2457382.279\pm0.488$&2459986.476263&TOI-586\\
5695996352497664512&$121.78925\pm0.19501$&$0.07\pm0.02$&$29.6\pm21.5$&$16.603\pm$&$2457422.893\pm7.351$&2459974.937344&TOI-592\\
4641589646622686720&$13.71695\pm0.00828$&$0.13\pm0.08$&$167.4\pm13.4$&$18.642\pm0.422$&$2457388.81\pm0.471$&2459184.759271&TOI-646\\
5417424326998593408&$14.06688\pm0.00123$&$0.25\pm0.01$&$90.2\pm2.6$&$12.334\pm0.125$&$2457393.464\pm0.102$&2458547.303252&TOI-665\\
5416752486737577984&$4.37836\pm0.00033$&$0.04\pm0.04$&$196.5\pm59.6$&$17.741\pm0.689$&$2457387.874\pm0.71$&2459283.065609&TOI-668\\
5395959695358663296&$4.21329\pm0.00102$&$0.09\pm0.09$&$241.7\pm70.5$&$11.395\pm1.044$&$2457390.043\pm0.811$&2459331.163575&TOI-759\\
6161800502228330240&$7.62315\pm0.00256$&$0.04\pm0.02$&$182.2\pm34.5$&$35.183\pm0.342$&$2457384.731\pm0.802$&2459319.912483&TOI-838\\
4916461712411594112&$14.20745\pm0.00218$&$0.28\pm0.03$&$337.2\pm7.7$&$26.282\pm1.382$&$2457384.774\pm0.275$&2458363.76296&TOI-846\\
5925532800797072128&$3.231\pm0.00003$&$0.05\pm0.01$&$109.7\pm7.6$&$49.749\pm0.338$&$2457387.738\pm0.067$&2459362.247825&TOI-901\\
4769649280577737728&$12.12195\pm0.00414$&$0.33\pm0.04$&$68.6\pm9.3$&$24.069\pm1.326$&$2457382.988\pm0.367$&2459373.317914&TOI-924\\
2961066353557939456&$12.71088\pm0.00065$&$0.34\pm0.01$&$334.6\pm1.4$&$33.552\pm0.309$&$2457387.801\pm0.043$&2458442.13529&TOI-948\\
3285409673726608768&$2.96835\pm0.00011$&$0.06\pm0.02$&$341.1\pm15.9$&$16.529\pm0.272$&$2457389.074\pm0.13$&2458441.29935&TOI-953\\
5714269239318650880&$14.53957\pm0.00219$&$0.33\pm0.01$&$286.8\pm3$&$33.698\pm0.569$&$2457389.649\pm0.092$&2458494.77797&TOI-996\\

5505717481529404416&$4.95921\pm0.00035$&$0.05\pm0.03$&$70\pm33.6$&$35.909\pm1.946$&$2457386.116\pm0.454$&2458492.78078&TOI-1018\\
5911682531996474624&$9.44988\pm0.00044$&$0.16\pm0.01$&$117.7\pm3.6$&$21.494\pm0.163$&$2457384.907\pm0.103$&2459378.714316&TOI-1059\\
4649937757389347456&$12.85107\pm0.00529$&$0.14\pm0.05$&$232.3\pm28.6$&$17.411\pm1.121$&$2457393.393\pm1.005$&2459211.732146&TOI-1072\\
6445176465824182272&$11.47501\pm0.00037$&$0.3\pm0.01$&$48\pm1.2$&$46.241\pm0.305$&$2457387.988\pm0.035$&2460131.889805&TOI-1111\\
6650192366014887424&$4.45273\pm0.00015$&$0.47\pm0.03$&$222.6\pm1.9$&$54.062\pm2.875$&$2457388.533\pm0.014$&2458658.32747&TOI-1115\\
6660655834058823680&$10.95889\pm0.0008$&$0.25\pm0.01$&$207.4\pm4$&$38.762\pm0.662$&$2457393.581\pm0.111$&2458666.52199&TOI-1119\\
1421127098253596288&$13.743\pm0.00112$&$0.18\pm0.01$&$346\pm3.7$&$15.273\pm0.176$&$2457390.682\pm0.135$&2459400.983335&TOI-1140\\
1726947014749701504&$6.03613\pm0.00008$&$0.02\pm0.01$&$1.3\pm14.2$&$43.790\pm0.254$&$2457385.844\pm0.237$&2459759.99969&TOI-1153\\
1635325672880724864&$11.24634\pm0.00104$&$0.04\pm0.02$&$333.3\pm32.6$&$11.169\pm0.301$&$2457383.722\pm1.016$&2459817.020033&TOI-1186\\
2160710158704303360&$5.96192\pm0.0013$&$0.13\pm0.08$&$327.6\pm35.4$&$10.404\pm0.644$&$2457389.331\pm0.625$&2459759.178675&TOI-1251\\
2289068176923197952&$14.30135\pm0.00522$&$0.22\pm0.05$&$99.6\pm12$&$12.083\pm0.548$&$2457385.169\pm0.44$&2459695.445887&TOI-1270\\
2246355002042750976&$3.62345\pm0.00023$&$0.02\pm0.04$&$144.9\pm69.8$&$15.306\pm0.411$&$2457388.368\pm0.699$&2459852.060009&TOI-1455\\
348551718652896000&$5.93844\pm0.00046$&$0.03\pm0.03$&$126.5\pm61$&$29.933\pm0.951$&$2457390.826\pm0.979$&2459908.543488&TOI-1553\\
443040655569966208&$17.32247\pm0.0012$&$0.34\pm0.01$&$186.4\pm1.5$&$30.281\pm0.529$&$2457385.245\pm0.06$&2458808.52242&TOI-1567\\
352678495029040000&$17.33133\pm0.00533$&$0.11\pm0.03$&$62.4\pm20.9$&$29.951\pm0.913$&$2457396.587\pm1.078$&2458794.15217&TOI-1572\\
462926457230782208&$51.92655\pm0.12469$&$0.27\pm0.08$&$338\pm16$&$16.763\pm13.32$&$2457408.923\pm2$&2458807.93693&TOI-1591\\
957955110633719552&$8.52111\pm0.00129$&$0.17\pm0.03$&$354.3\pm14.1$&$37.860\pm1.585$&$2457388.177\pm0.334$&2458847.69726&TOI-1698\\
1039196547341014016&$9.57303\pm0.00051$&$0.38\pm0.01$&$236.4\pm1.6$&$31.935\pm0.470$&$2457385.971\pm0.035$&2458851.5904&TOI-1786\\
802616348383896448&$8.70492\pm0.00032$&$0.42\pm0.01$&$331.4\pm1$&$51.475\pm0.401$&$2457391.073\pm0.021$&2459627.995561&TOI-1787\\
751544445585226496&$5.34341\pm0.00025$&$0.02\pm0.02$&$103.7\pm60.6$&$19.850\pm0.585$&$2457389.28\pm0.901$&2458875.04671&TOI-1788\\
1602005522755589760&$98.5329\pm0.22629$&$0.2\pm0.04$&$279\pm9.9$&$14.466\pm0.564$&$2457352.355\pm2.515$&2459517.338757&TOI-1856\\
548075249022607744&$48.54992\pm0.04997$&$0.24\pm0.02$&$8\pm6.8$&$12.412\pm0.364$&$2457390.782\pm1.021$&2459000.999918&TOI-1897\\
5199893510584259968&$4.82955\pm0.00102$&$0.17\pm0.06$&$78.1\pm19$&$13.101\pm0.944$&$2457386.224\pm0.238$&2459381.402207&TOI-1951\\
5235114127904811648&$5.43772\pm0.00029$&$0.01\pm0.02$&$29.4\pm108.4$&$42.067\pm0.634$&$2457389.71\pm1.641$&2459354.324182&TOI-1974\\
5348534425968598400&$6.65906\pm0.00119$&$0.07\pm0.06$&$31.3\pm26$&$9.571\pm0.280$&$2457387.231\pm0.465$&2460065.075037&TOI-1991\\
5377428178491618944&$15.44476\pm0.00876$&$0.18\pm0.06$&$28.8\pm22$&$8.454\pm0.591$&$2457384.532\pm0.889$&2458576.4335&TOI-1996\\
5096613016130459136&$51.62784\pm0.0394$&$0.24\pm0.01$&$277.9\pm2.3$&$14.884\pm0.144$&$2457368.6\pm0.341$&2459178.169&TOI-2008\\
2295415623189777024&$3.73216\pm0.00039$&$0.14\pm0.12$&$281.2\pm28$&$12.911\pm1.382$&$2457388.248\pm0.264$&2459913.435645&TOI-2038\\
4570820611494681984&$8.42351\pm0.00158$&$0.18\pm0.03$&$172\pm7.9$&$13.627\pm0.429$&$2457389.474\pm0.187$&2459764.110052&TOI-2157\\
5689821044216119296&$11.56211\pm0.007$&$0.22\pm0.08$&$177.9\pm22$&$13.359\pm0.962$&$2457384.105\pm0.666$&2459268.759188&TOI-2349\\
4671762272913404160&$22.85492\pm0.02846$&$0.17\pm0.14$&$326\pm44.1$&$8.544\pm1.087$&$2457398.755\pm2.39$&2459073.99562&TOI-2360\\
3023791185522078592&$17.17497\pm0.00886$&$0.24\pm0.03$&$235.4\pm8.4$&$22.478\pm0.877$&$2457384.697\pm0.394$&2459224.966718&TOI-2366\\
6825245573613327616&$13.41891\pm0.00521$&$0.02\pm0.05$&$119.4\pm108.6$&$21.864\pm0.923$&$2457383.762\pm4.058$&2459066.937927&TOI-2413\\
4884422424614580352&$17.11766\pm0.00585$&$0.24\pm0.03$&$93.1\pm5.8$&$22.112\pm0.551$&$2457393.51\pm0.309$&2459183.305376&TOI-2442\\
3173208463482530176&$2.37813\pm0.00015$&$0.16\pm0.05$&$154\pm18.6$&$19.225\pm1.450$&$2457389.291\pm0.123$&2459198.809559&TOI-2469\\
3321419774751152128&$10.09911\pm0.00768$&$0.08\pm0.13$&$130.4\pm59.1$&$12.578\pm0.982$&$2457384.436\pm1.676$&2459202.053965&TOI-2492\\
1259922196651254272&$6.69241\pm0.00481$&$0.2\pm0.13$&$69.7\pm31.2$&$7.388\pm1.105$&$2457387.977\pm0.615$&2459682.185785&TOI-2533\\
5320246568758675328&$21.05714\pm0.00615$&$0.06\pm0.02$&$3.7\pm30.3$&$29.625\pm0.652$&$2457392.621\pm1.735$&2459284.317234&TOI-2544\\
5697796768432105216&$8.02433\pm0.00188$&$0.43\pm0.04$&$47.3\pm10.9$&$12.999\pm0.813$&$2457387.293\pm0.238$&2459233.496293&TOI-2555\\
3026047834355902464&$5.73382\pm0.00061$&$0.11\pm0.02$&$89\pm10.3$&$50.019\pm0.881$&$2457391.279\pm0.152$&2459226.801169&TOI-2598\\
5301643549272386560&$1.4508\pm0.0001$&$0.05\pm0.11$&$141.9\pm126.5$&$18.377\pm2.461$&$2457389.055\pm0.499$&2459330.683649&TOI-2606\\
3855170410190523008&$3.96011\pm0.00011$&$0.03\pm0.02$&$127\pm15.1$&$46.699\pm0.494$&$2457386.832\pm0.166$&2459275.974283&TOI-2664\\
3166138805578006016&$4.39132\pm0.00064$&$0.08\pm0.06$&$354.8\pm24.6$&$50.548\pm1.432$&$2457389.978\pm0.297$&2459222.51667&TOI-2819\\
5310692633056834432&$8.61119\pm0.00119$&$0.08\pm0.02$&$127.5\pm13.4$&$50.991\pm0.958$&$2457388.438\pm0.319$&2459989.197536&TOI-3006\\
5299710470390857728&$9.54298\pm0.00159$&$0.36\pm0.05$&$72\pm12.4$&$18.911\pm1.885$&$2457387.876\pm0.25$&2459318.200838&TOI-3010\\
5202007248674569728&$4.28108\pm0.00042$&$0.08\pm0.05$&$9.8\pm46.8$&$22.504\pm1.308$&$2457387.087\pm0.528$&2459387.985248&TOI-3148\\
5869945139392446336&$4.64947\pm0.00063$&$0.07\pm0.04$&$256.3\pm33.5$&$11.737\pm0.436$&$2457390.276\pm0.437$&2459355.282092&TOI-3155\\
5851691833256275200&$8.87867\pm0.00136$&$0.05\pm0.04$&$120.7\pm31.3$&$63.511\pm2.292$&$2457386.336\pm0.746$&2459355.803726&TOI-3191\\
6070306974290936960&$6.83559\pm0.002$&$0.11\pm0.06$&$188.8\pm32.6$&$15.931\pm0.850$&$2457390.354\pm0.628$&2459351.726265&TOI-3241\\
4639398560466507904&$11.45074\pm0.0026$&$0.26\pm0.05$&$310.6\pm14.5$&$23.482\pm1.558$&$2457384.716\pm0.419$&2459365.448337&TOI-3260\\
6419210296144773504&$3.05342\pm0.00025$&$0.11\pm0.06$&$118.8\pm22.5$&$41555\pm2075$&$2457388.216\pm0.184$&2459388.724951&TOI-3298\\
3486043573401367168&$15.34617\pm0.00528$&$0.05\pm0.03$&$143.4\pm30.3$&$13.900\pm0.323$&$2457380.934\pm1.292$&2459313.471423&TOI-3501\\
5343051878733534592&$3.44688\pm0.00052$&$0.07\pm0.07$&$163.5\pm116.3$&$23.342\pm3.010$&$2457387.712\pm1.107$&2459307.388819&TOI-3502\\
2057752233480414848&$4.20558\pm0.00116$&$0.14\pm0.07$&$249.9\pm34.5$&$13.089\pm0.891$&$2457390.293\pm0.386$&2459813.403681&TOI-3542\\
189461074831319680&$4.42384\pm0.00028$&$0.08\pm0.03$&$61.1\pm19$&$55.274\pm1.936$&$2457390.179\pm0.225$&2459912.449974&TOI-3756\\
1087913090069066496&$14.99837\pm0.00239$&$0.3\pm0.02$&$80.8\pm6.5$&$21.055\pm0.563$&$2457385.255\pm0.216$&2458849.115258&TOI-3796\\
1512692949146107520&$10.15982\pm0.00103$&$0.02\pm0.02$&$64.9\pm46.4$&$36.145\pm0.760$&$2457387.776\pm1.32$&2459675.336571&TOI-3904\\
6063252821253530752&$7.49949\pm0.0006$&$0.01\pm0.01$&$153.8\pm67.1$&$28.259\pm0.420$&$2457386.703\pm1.398$&2459350.811013&TOI-4338\\
6463801879263478144&$7.06131\pm0.00179$&$0.07\pm0.06$&$313\pm59.3$&$14.282\pm1.307$&$2457389.798\pm1.173$&2459038.946551&TOI-4400\\
4605954852723545088&$4.91455\pm0.00092$&$0.13\pm0.06$&$213.4\pm24.6$&$9.731\pm0.462$&$2457388.057\pm0.34$&2459789.419251&TOI-4462\\
2395520590619923328&$8.11076\pm0.00092$&$0.06\pm0.03$&$325.9\pm34.6$&$42.944\pm1.390$&$2457388.802\pm0.779$&2459104.0983&TOI-4657\\
577614689757449728&$8.44816\pm0.00078$&$0.01\pm0.01$&$80.8\pm86.5$&$32.950\pm0.547$&$2457384.963\pm2.03$&2459235.815084&TOI-4792\\
5587000905841875456&$17.68939\pm0.01404$&$0.43\pm0.06$&$194.9\pm6.6$&$25.073\pm3.242$&$2457386.372\pm0.365$&2459245.196258&TOI-4807\\
5230545317792027776&$7.94833\pm0.0006$&$0.04\pm0.03$&$324.6\pm29.5$&$23.257\pm0.466$&$2457387.46\pm0.65$&2459354.079175&TOI-4973\\
600788374781198720&$4.98999\pm0.00033$&$0.06\pm0.04$&$45.8\pm23.4$&$59.118\pm1.320$&$2457388.337\pm0.332$&2457140.02&TOI-5103\\
2167586710592820096&$27.3883\pm0.0198$&$0.33\pm0.05$&$343.7\pm10$&$8.449\pm0.497$&$2457400.551\pm0.63$&2459814.873357&TOI-5149\\
3278323493085459456&$22.85312\pm0.01706$&$0.28\pm0.05$&$241.7\pm6.3$&$13.571\pm0.553$&$2457385.682\pm0.406$&2459489.758703&TOI-5156\\
1130631384551617024&$20.57286\pm0.00427$&$0.54\pm0.02$&$217.7\pm3.7$&$31.281\pm1.035$&$2457385.098\pm0.137$&2459588.291193&TOI-5157\\
2148571309814936576&$17.43558\pm0.00715$&$0.15\pm0.03$&$267.9\pm13.4$&$28.589\pm0.984$&$2457393.599\pm0.656$&2459887.497008&TOI-5200\\
2581395161599229952&$5.29846\pm0.00032$&$0.04\pm0.02$&$347.9\pm22$&$65.256\pm0.918$&$2457388.296\pm0.325$&2459490.963737&TOI-5307\\
109773424146717568&$11.63028\pm0.00448$&$0.19\pm0.07$&$333.9\pm10.4$&$50.553\pm5.427$&$2457387.128\pm0.311$&2459513.585855&TOI-5372\\
983011056484954496&$12.74426\pm0.00116$&$0.39\pm0.02$&$265.2\pm2$&$33.531\pm0.685$&$2457393.503\pm0.077$&2459942.544324&TOI-5379\\
623779716969345920&$15.19502\pm0.00145$&$0.29\pm0.01$&$246.3\pm2.3$&$27.427\pm0.209$&$2457388.115\pm0.138$&2459561.627836&TOI-5394\\
3429797609407986176&$10.05227\pm0.00222$&$0.16\pm0.04$&$82.7\pm19.8$&$49.723\pm2.538$&$2457388.303\pm0.532$&2459540.386039&TOI-5475\\
674670853180191360&$19.63351\pm0.00293$&$0.39\pm0.07$&$296.1\pm3.7$&$26.115\pm2.565$&$2457396.405\pm0.135$&2459516.534272&TOI-5547\\
3643353863081886336&$3.84803\pm0.00012$&$0.03\pm0.03$&$264.7\pm21.4$&$31.300\pm0.363$&$2457387.413\pm0.24$&2459694.827263&TOI-5627\\
1018729069670619520&$24.56862\pm0.01622$&$0.11\pm0.05$&$285.5\pm22.6$&$8.364\pm490$&$2457383.636\pm1.543$&2458891.862067&TOI-5746\\
548058859427458688&$19.54594\pm0.00435$&$0.02\pm0.02$&$223.9\pm42.2$&$35.368\pm0.542$&$2457393.799\pm2.285$&2459722.313637&TOI-5761\\
1802021977935667200&$5.2484\pm0.00076$&$0.33\pm0.1$&$192.8\pm11.4$&$28.068\pm5.094$&$2457387.209\pm0.147$&2459795.355448&TOI-5860\\
1869489729418662528&$7.15108\pm0.00328$&$0.14\pm0.11$&$155.5\pm55.9$&$2.379\pm0.284$&$2457389.351\pm1.049$&2459818.905315&TOI-5882\\
2070280099026014336&$5.83283\pm0.00052$&$0.06\pm0.02$&$309.8\pm22.3$&$58.051\pm1.268$&$2457389.883\pm0.351$&2459848.780642&TOI-6111\\
2838654459861938944&$9.86148\pm0.01254$&$0.07\pm0.14$&$22.3\pm128.9$&$6.618\pm0.867$&$2457391.848\pm3.435$&2459850.257269&TOI-6117\\
1928695681777800960&$3.65272\pm0.0004$&$0.06\pm0.04$&$67.8\pm40.8$&$19.284\pm1.029$&$2457387.344\pm0.423$&2459850.633702&TOI-6133\\
2871631592420978432&$9.76641\pm0.00417$&$0.22\pm0.06$&$277.3\pm25.8$&$12.499\pm0.962$&$2457384.562\pm0.651$&2459881.332399&TOI-6207\\
392652614647892736&$5.15542\pm0.00088$&$0.11\pm0.07$&$274.1\pm40.1$&$9.571\pm0.826$&$2457389.59\pm0.567$&2459878.34576&TOI-6218\\
2859788722613818112&$5.6036\pm0.0011$&$0.03\pm0.07$&$182.5\pm111.3$&$9.379\pm0.831$&$2457387.542\pm1.741$&2459879.464465&TOI-6242\\
6057181524220247680&$17.43205\pm0.01431$&$0.49\pm0.05$&$74.3\pm11.9$&$9.735\pm0.568$&$2457383.109\pm0.573$&2460068.759071&TOI-6568\\
5795018365391402368&$6.56902\pm0.00308$&$0.11\pm0.14$&$173.3\pm43.3$&$11.197\pm1.067$&$2457391.649\pm0.795$&2460111.963815&TOI-6611\\

\vspace{-0.3cm}
\enddata
\tablecomments{New EBs Matches between Gaia DR3 NSS SB1 and candidate transiting planet systems.}
\end{deluxetable*}
\clearpage
